On the Reliability Function of the Discrete Memoryless Relay Channel

Bounds on the reliability function for the discrete memoryless relay channel are derived using the method of types. Two achievable error exponents are derived based on partial decode-forward and compress-forward which are well-known superposition block-Markov coding schemes. The derivations require combinations of the techniques involved in the proofs of Csisz\'ar-K\"orner-Marton's packing lemma for the error exponent of channel coding and Marton's type covering lemma for the error exponent of source coding with a fidelity criterion. The decode-forward error exponent is evaluated on Sato's relay channel. From this example, it is noted that to obtain the fastest possible decay in the error probability for a fixed effective coding rate, one ought to optimize the number of blocks in the block-Markov coding scheme assuming the blocklength within each block is large. An upper bound on the reliability function is also derived using ideas from Haroutunian's lower bound on the error probability for point-to-point channel coding with feedback.

==> decode.tex <==
\section{Partial Decode-Forward (PDF)}\label{sec:dec}

We warm up by deriving two achievable error exponents using PDF. In  PDF, the relay decodes part of the message in each block. For block $j\in [b]$, the part of the message that is decoded by the relay is indicated as $M_j'$ and the remainder of the message  is $M_j''$. Thus, $M_j = (M_j', M_j'')$.  We will state the theorems in Sections~\ref{sec:pdf} and~\ref{sec:expurga}. The key lemma to prove these theorems is the packing lemma for relaying which is stated in Section~\ref{sec:pack}. Proofs of these results are presented in Sections~\ref{prf:pdf} and~\ref{prf:expu}.

\subsection{Analogue of the Random Coding Error Exponent} \label{sec:pdf}
By generalizing the packing lemmas in Haroutunian {\em et al.} \cite{Har08} and K\"orner-Sgarro~\cite{Kor80b} and using MMI decoding~\cite{Goppa}, we obtain the following analogue of the random coding error exponent:
\begin{theorem}[Random Coding Error Exponent for Relaying]  \label{thm:pdf}
Fix $b\in\bbN$,  auxiliary alphabet $\calU$ and a joint  distribution $Q_{X_2}\times  Q_{U|X_2} \times   Q_{X_1|U X_2}\in\scP(\calX_2\times\calU\times\calX_1)$. These distributions induce the following virtual channels:
\begin{align}
W_{Y_2|U X_2}(y_2|u,x_2) &:=\sum_{x_1,y_3} W(y_2,y_3|x_1,x_2)Q_{X_1|U X_2}(x_1|u, x_2) \label{eqn:vir1}\\
W_{Y_3|U X_2}(y_3|u,x_2) &:=  \sum_{x_1,y_2} W(y_2,y_3|x_1,x_2)Q_{X_1|U X_2}(x_1|u, x_2) \label{eqn:vir2}\\
W_{Y_3|U X_1 X_2} (y_3|u,x_1,x_2) & :=\sum_{y_2} W(y_2,y_3|x_1,x_2) . \label{eqn:vir3}
\end{align}
We have the following lower bound on $E_b(\Reff)$:
\begin{eqnarray}
E_b(\Reff)  \ge \frac{1}{b} \left[ \max_{R'+R''=R}\min\{F(R'), G (R'),  \tilG(R'')\} \right],  \label{eqn:pdf_lb}
\end{eqnarray}
where $F(R'), G(R' )$ and  $\tilG(R'')$ are  constituent error exponents defined as 
\begin{align}
F(R')&:=\min_{V:\calU\times\calX_2\to\calY_2}D(V\|W_{Y_2|U X_2}|Q_{U X_2})  + \left|  I(Q_{U|X_2},V|Q_{X_2})-R' \right|^+  \label{eqn:F}\\
G(R')&:=\min_{V:\calU\times\calX_2\to\calY_3}D(V\|W_{Y_3|U X_2}|Q_{U X_2})  +\left|    I(Q_{ U , X_2},V)-R'  \right|^+ \label{eqn:G1}\\
 \tilG(R'')&:= \min_{V:\calU\times\calX_1\times\calX_2\to\calY_3}  D(V\|W_{Y_3|U X_1 X_2}|Q_{U X_2 X_1} ) +\left|   I(Q_{X_1|U X_2},V|Q_{U X_2})-R''  \right|^+  \label{eqn:G2}
\end{align}
\end{theorem}
The proof of this result is based on a modification of the packing lemma and is provided in Section~\ref{prf:pdf}. 

A few comments are in order with regard to Theorem~\ref{thm:pdf}.
Firstly, since $Q_{X_2}$, $Q_{U|X_2}$ and $Q_{X_1| U X_2}$ as well as the splitting of $R$ into $R'$ and $R''$  are arbitrary, we can maximize the lower bounds in \eqref{eqn:pdf_lb}   over these free parameters.    Secondly, for a fixed split $R'+R''=R$, if 
\begin{align}
R' &<  I(U  ;Y_2|X_2) \\
R' &< I(U X_2;Y_3 )\\
R'' &< I( X_1;Y_3|U X_2),
\end{align}
for some $Q_{X_2}$, $Q_{U|X_2}$ and $Q_{X_1| U X_2}$, then $F(R')$, $G(R')$ and $\tilG(R'')$ are positive.   Hence, the error probability decays exponentially fast if $R$ satisfies the PDF lower bound in~\eqref{eqn:cap_pdf}.  Note that $F(R')$ is the error exponent  for decoding a part of the message at the relay and $G(R')$  and $\tilG(R'')$  are the error exponents for decoding the rest of the message at the decoder.  Setting $U=X_1$ recovers DF for which the error exponent is provided in~\cite{Bra12}. Note that~\eqref{eqn:pdf_lb}   demonstrates a tradeoff between the effective rate and error probability: for a fixed $R$, as the number of blocks $b$ increases, $\Reff$ increases but the lower bound  on the error exponent decreases.  Varying $R$ also, of course, allows us to observe  this tradeoff.% between the effective rate and error probability.

\subsection{Analogue of the Expurgated Error Exponent} \label{sec:expurga}
Now, for any stochastic matrix $V:\calU\times\calX\to\calY$, define the  {\em conditional Bhattacharyya distance}
\begin{equation}
\rvd_V(u,u'|x) := -\log\sum_y \sqrt{ V(y|u,x)V(y|u',x) } \label{eqn:bha} .
\end{equation} 
We also obtain the following improvement of the random coding bound known as the expurgated error exponent:
\begin{theorem}[Expurgated Error Exponent for Relaying]  \label{thm:expurate}
Fix $b\in\bbN$,  auxiliary alphabet $\calU$ and a joint  distribution $Q_{X_2}\times  Q_{U|X_2} \times   Q_{X_1|U X_2}\in\scP(\calX_2\times\calU\times\calX_1)$. These distributions induce the   virtual channels  in~\eqref{eqn:vir1}--\eqref{eqn:vir3}.  We have the following lower bound on $E_b(\Reff)$:
\begin{eqnarray}
E_b(\Reff)  \ge \frac{1}{b} \left[ \max_{R'+R''=R}\min\{F_\rmx(R'), G_\rmx(R'),  \tilG_\rmx(R'')\} \right],  \label{eqn:pdf_lb_ex}
\end{eqnarray}
where $F_\rmx(R'), G_\rmx(R' )$ and  $\tilG_\rmx(R'')$ are  constituent error exponents defined as 
\begin{align}
F_\rmx(R') &:= \min_{ \substack{ P_{U U'|X_2} : P_{U|X_2}=P_{U'|X_2} = Q_{U|X_2}\\ I(P_{U|X_2}, P_{U'|U X_2} |Q_{X_2})\le R'}} \bbE   \left[ \rvd_{W_{Y_2|U,X_2}} (U,U'|X_2) \right] + I(P_{U|X_2}, P_{U'|U X_2} |Q_{X_2})-R' \label{eqn:Fx}\\
G_\rmx(R') &:= \min_{ \substack{ P_{U  X_2  U'  X_2' } : P_{U X_2}=P_{U' X_2'} = Q_{U   X_2}\\ I(P_{U X_2}, P_{U' X_2' | U X_2}  ) \le R'}} \bbE   \left[ \rvd_{W_{Y_3|U X_2}} (UX_2,U'X_2' ) \right] + I(P_{U X_2}, P_{U' X_2' | U X_2}  )-R' \label{eqn:Gx}\\
\tilG_\rmx(R') &:= \min_{ \substack{ P_{X_1 X_1'|U  X_2   } : P_{X_1 |U  X_2   } =P_{ X_1'|U  X_2   }  = Q_{X_1|U   X_2}\\  I(P_{X_1  |U  X_2   } , P_{X_1'|U  X_2  X_1  }| Q_{U X_2})  \le R''}} \bbE   \left[ \rvd_{W_{Y_3|U X_1 X_2}} (X_1,X_1' |U X_2) \right]  \nn\\
 & \qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad +  I(P_{X_1  |U  X_2   } , P_{X_1'|U  X_2  X_1  }| Q_{U X_2})-R'' \label{eqn:Gxtil}
\end{align}
\end{theorem}
The proof of this result is based on a generalization of the packing lemma and is provided in Section~\ref{prf:expu}.  Note that unlike the analogue of the random coding exponent, the decoder used in the proof of the expurgated exponent is maximum-likelihood-based and hence, the exponent is  not universally attainable.

Note that each of the expectations in \eqref{eqn:Fx}, \eqref{eqn:Gx} and \eqref{eqn:Gxtil} is taken with respect to the optimization variable and the fixed distributions $Q_{X_1},  Q_{U|X_2}$ and $Q_{X_1|U X_2}$. For example in \eqref{eqn:Fx}, 
\begin{align}
 \bbE   \left[ \rvd_{W_{Y_2|U,X_2}} (U,U'|X_2) \right] &=\sum_{u,u',x_2} P_{U U'|X_2}(u,u'|x_2) Q_{X_2}(x_2) \rvd_{W_{Y_2|U,X_2}} (u,u'|x_2) %\\
% I(U;U'|X_2) & = I(P_{U|X_2}, P_{U'|U X_2} |Q_{X_2})
\end{align}
The interpretation of the expurgated bound is similar to the random coding bound. In fact, it has long been known~\cite[Prob.\ 10.18(c)]{Csi97} that the expurgated bound is no smaller than the random coding bound. Hence, if $R$ satisfies the PDF lower bound in~\eqref{eqn:cap_pdf}, then the lower bound in \eqref{eqn:pdf_lb_ex} is positive and the error probability decays exponentially.


\subsection{Analogue of the  Packing Lemma  for Relaying} \label{sec:pack}
The proofs of Theorem~\ref{thm:pdf} and \ref{thm:expurate} use    generalizations of the  packing lemmas in~\cite{Har08}. We use the same coding structure and notations for the codewords as given in the book by El Gamal and Kim~\cite[Thm.~16.3]{elgamal}. In addition, for    $V,\hatV:\calU\times\calX_2\to\calY_2$, define $r_{V,\hatV}(m_j'|m_{j-1}')$  to be the fraction of $\calT_{V}( u^n(m_j'|m_{j-1}') , x_2^n(m_{j-1}'))$ that intersects with $\hatV$-shells of $(u^n(\tilm_j'|m_{j-1}'),x_2^n(m_{j-1}'))$ for some $\tilm_j\ne m_j$, i.e., 
\begin{equation}
  r_{V,\hatV}(m_j'|m_{j-1}'):=\frac{\displaystyle \bigg|\calT_{V}( u^n(m_j'|m_{j-1}') , x_2^n(m_{j-1}')) \bigcap\bigcup_{\tilm_j'\ne m_j'}\calT_{ \hatV}( u^n(\tilm_j'|m_{j-1}') , x_2^n(m_{j-1}'))  \bigg|}{ \left| \calT_{V}( u^n(m_j'|m_{j-1}') , x_2^n(m_{j-1}')) \right| } \label{eqn:defr}
\end{equation}
 Similarly, for  $V,\hatV:\calU\times\calX_2\to\calY_3$, define   $s_{V,\hatV}(m_{j+1}'|m_{j}')$   to be  the fraction of $\calT_V(u^n(m_{j+1}'|m_j'), x_2^n(m_j'))$ that intersects with $\hatV$-shells of $(u^n(m_{j+1}'|\tilm_{j}'),x_2^n(\tilm_{j}'))$ for some $\tilm_{j}'\ne m_j'$, i.e., 
\begin{equation}
s_{V,\hatV}(m_{j+1}'|m_{j}'):= \frac{\displaystyle  \bigg|\calT_V(u^n(m_{j+1}'|m_j'), x_2^n(m_j')) \bigcap\bigcup_{\tilm_j'\ne m_j'} \calT_{\hatV}(u^n(m_{j+1}'|\tilm_j'), x_2^n(\tilm_j'))  \bigg| }{ \left|\calT_V(u^n(m_{j+1}'|m_j'), x_2^n(m_j'))\right|} \label{eqn:defs}
\end{equation} 
  Lastly,  for  $V,\hatV: \calX_1\times\calX_2\times \calU\to\calY_3$, define   $t_{V,\hatV}(m_j''|m_j', m_{j-1}')$ to be the fraction of   $\calT_V( x_1^n(m_j', m_j''|m_{j-1}')$, $ x_2^n(m_{j-1}'), u^n(m_{j}'| m_{j-1}') )$   that intersects with $\hatV$-shells of $(x_1^n(m_j', \tilm_j''|m_{j-1}'), x_2^n(m_{j-1}'), u^n(m_{j}'| m_{j-1}'))$ for some $\tilm_j''\ne m_j''$, i.e.,
\begin{align}
&t_{V,\hatV}(m_j''|m_j', m_{j-1}') \nn\\*
 & := \frac{ \displaystyle    \bigg|\calT_V( x_1^n(m_j', m_j''|m_{j-1}'),  x_2^n(m_{j-1}'), u^n(m_{j}'| m_{j-1}') )\bigcap\bigcup_{\tilm_j'' \ne m_j''} \calT_{\hatV}( x_1^n(m_j', \tilm_j''|m_{j-1}'),  x_2^n(m_{j-1}'), u^n(m_{j}'| m_{j-1}') )  \bigg| }{\left|\calT_V( x_1^n(m_j', m_j''|m_{j-1}'),  x_2^n(m_{j-1}'), u^n(m_{j}'| m_{j-1}') ) \right|} \label{eqn:deft}
\end{align}  
With these definitions, we can state the packing lemma for PDF.


\begin{lemma}[Packing Lemma for Relaying]   \label{lem:packing_df}
Fix  $\delta>0$ and nonnegative numbers   $(R',R'')$ such that $R',R''>\delta$. For every $j \in [b]$, and for every joint type $Q_{X_2}\times Q_{U|X_2} \times Q_{X_1|U X_2} \in \scP_n(\calX_2\times\calU\times\calX_1)$ satisfying $H(Q_{X_2})<R'$, $H(Q_{U|X_2}|Q_{X_2}) < R'$ and $H(Q_{X_1 | U X_2} | Q_{U| X_2} Q_{X_2}) <R''$, there exists at least $\exp( n (R' - \delta) )$  sequences $(x_2^n(m_{j-1}'), u^n(m_j'|m_{j-1}')) \in \calT_{Q_{X_2} \times Q_{U|X_2}} $  and for every $(m_j',m_{j-1}') \in [\exp( n (R' - \delta) )]^2$ at least $\exp( n (R''-\delta))$ sequences $x_1^n(m_j', m_j''|m_{j-1}')\in \calT_{Q_{X_1|U X_2}}(  u^n(m_j'|m_{j-1}'), x_2^n(m_{j-1}'))$ such that for  all sufficiently large $n>n_0(\delta,b, |\calU|, |\calX_1|,  |\calX_2|, |\calY_2|, |\calY_3| )$, the following hold:
\begin{enumerate}
\item For every $V ,\hatV :\calU\times\calX_2\to\calY_2$, and every $m_j'$,
\begin{align}
r_{V ,\hatV }(m_j'|m_{j-1}') \le  \exp(-n |  \,  I(Q_{U|X_2},\hatV |Q_{X_2})-R'   | ^+ ), \label{eqn:rvv}
\end{align}
\item For every $V ,\hatV :\calU\times\calX_2\to\calY_3$,  and every $m_j'$,
\begin{equation}  
s_{V ,\hatV }(m_{j+1}'|m_{j}')\le  \exp(-n | \,  I(Q_{X_2}Q_{U|X_2},\hatV )-R'  | ^+ ), \label{eqn:svv}
\end{equation}
\item For every $V ,\hatV :\calU\times\calX_1\times\calX_2\to\calY_3$, and every $m_j''$, 
\begin{equation}
t_{V ,\hatV }(m_j''|m_j', m_{j-1}')\le \exp(- n | I(Q_{X_1|U X_2},\hatV | Q_{U X_2})-R''  | ^+ ) . \label{eqn:tvv}
\end{equation}\end{enumerate}
\end{lemma}
This lemma is proved in Appendix~\ref{app:pack}. 

\subsection{Proof of  Theorem~\ref{thm:pdf}} \label{prf:pdf}

\begin{proof}
We code over $b$ blocks each of length $n$ (block-Markov coding~\cite{CEG}). We fix a joint type $Q_{X_2}\times  Q_{U|X_2} \times   Q_{X_1|U X_2}  \in \scP_n(\calX_2\times\calU\times\calX_1)$.  Split   each message $M_j , j\in[b-1]$ of rate $R$ into two independent parts  $M_j'$ and $M_j''$ of rates $R'$ and $R''$ respectively. Use the codebook provided in Lemma~\ref{lem:packing_df}. 
%The codebook for block $j\in [b]$ consists of constant composition codewords $(x_2^n(m_{j-1}'), u^n(m_j'|m_{j-1}') ) \in\calT_{Q_{X_2} Q_{U|X_2}}$  as well as conditionally constant composition codewords $x_1^n(m_j', m_j''|m_{j-1}')\in \calT_{Q_{X_1|U X_2}}(  u^n(m_j'|m_{j-1}'), x_2^n(m_{j-1}'))$.  
At the $j$-th step, the relay does MMI decoding~\cite{Goppa} for $m_j'$ given $m_{j-1}'$ and $y_2^n(j)$. More precisely, it declares that $\check{m}_j'$ is sent if 
\begin{align}
\check{m}_j' = \argmax_{m_j' \in [ \exp(n (R' -\delta) ) ] }  \hatI( u^n (m_j'|m_{j-1}') \wedge y_2^n(j) | x_2^n(m_{j-1}') ) . \label{eqn:relay_j}
\end{align}
By convention, set $m_0'=1$. Recall that $\hatI( u^n (m_j'|m_{j-1}') \wedge y_2^n(j) | x_2^n(m_{j-1}') )$ is the conditional mutual information $I(\tilU; \tilY_2| \tilX_2)$ where the dummy random variables $(\tilX_2, \tilU, \tilY_2)$ have joint type given by the sequences $(u^n (m_j'|m_{j-1}'), x_2^n(m_{j-1}'), y_2^n(j))$. 
%Here and in the following, if there is a tie that maximizes any objective function, let the chosen index be the smallest one.
After all blocks are received, the decoder performs backward decoding   using MMI~\cite{Goppa}.  In particular, it declares that $\hatm_{j}'$ is sent if 
\begin{equation}
\hatm_{j}' = \argmax_{m_j' \in [ \exp(n (R' -\delta) ) ]   }    \hatI( u^n (m_{j+1}'|m_{j}') , x_2^n(m_j')\wedge y_3^n(j) ) . \label{eqn:decoder_j}
\end{equation}
After all $\hatm_j', j\in [b-1]$ have been decoded in step~\eqref{eqn:decoder_j},  the decoder then decodes   $m_j''$    using MMI~\cite{Goppa}  as follows:
\begin{align}
\hatm_j''=\argmax_{m_j''\in[ \exp(n (R'' -\delta) ) ]  }   \hatI(   x_1^n(m_{j}', m_j''|m_{j-1}') \wedge y_3^n(j)     | \, u^n (m_{j}'|\hatm_{j-1}') , x_2^n(\hatm_{j-1}') ) \label{eqn:decoder_j2} .
 \end{align}
In steps~\eqref{eqn:relay_j}, \eqref{eqn:decoder_j} and \eqref{eqn:decoder_j2} if there exists more than one message attaining the $\argmax$, then pick any one uniformly at random. Note that since the code is of constant composition, MMI decoding is the same as minimum conditional entropy decoding~\cite{CK81}.  We assume, by symmetry, that $M_j=(M_j',M_j'')=(1,1)$ is sent for all $j\in[b - 1]$. The line of analysis in \cite[Sec.\ III]{Bra12} yields  % the following bound on the error probability:
\begin{equation} \label{eqn:union_bd}
\bbP(\hatM\ne M)\le (b-1) (\epsilon_{\rmR}+\epsilon_{\rmD,1} +\epsilon_{\rmD,2}) 
\end{equation}
where 
\begin{equation}
\epsilon_{\rmR}: =\bbP( \check{M}_j'\ne 1|\check{M}_{j-1}'= 1)
\end{equation}
 is the error probability  in relay decoding and 
\begin{align}
 \epsilon_{\rmD,1} &: = \bbP( \hatM_{j+1}'\ne 1| \hatM_{j+1}'=1, \check{M}_{j+1}=1), \quad \mbox{and}\\
    \epsilon_{\rmD,2}&:=\bbP( \hatM_{j}''\ne 1| \hatM_{j}'=1, \check{M}_{j-1}'=1)
\end{align} 
and are the error probabilities at the decoder. Since $b$ is assumed to be constant, it does not affect the exponential dependence of the error probability in \eqref{eqn:union_bd}. So we just bound $\epsilon_{\rmR}$, $\epsilon_{\rmD,1}$ and $\epsilon_{\rmD,2}$. Since all the calculations are similar, we   focus on
$\epsilon_\rmR$ leading to the error exponent $F(R')$ in \eqref{eqn:F}.
%$\epsilon_{\rmD,2}$.% leading to the error exponent $G_2(R'')$ in \eqref{eqn:G2}. 

An error occurs in step~\eqref{eqn:relay_j} (conditioned on neighboring blocks being decoded correctly so $\check{m}_{j-1}'={m}_{j-1}=1$) if and only if there exists $V,\hatV\in\scV_n(\calY_2; Q_{U|X_2} Q_{X_2})$ such that 
\begin{equation}
y_2^n(j) \in\calA_{V,\hatV}:= \calT_V(u^n(1 | 1) , x_2^n(1) ) \bigcap\bigcup_{\tilm_j' \ne 1}\calT_{\hatV}(u^n(\tilm_j' |1 ) , x_2^n( 1 ) ). \label{eqn:y3in}
\end{equation}
and 
\begin{equation}
I(Q_{U|X_2}, V|Q_{X_2})\le I(Q_{U|X_2}, \hatV|Q_{X_2}). \label{eqn:err_mmi} %Q_{X_1|UX_2}^n(x_1^n| u^n(1,1), x_2^n(1)) 
\end{equation}
Let the set of all $(V,V' )\in\scV_n(\calY_2; Q_{U|X_2} Q_{X_2})^2$ satisfying~\eqref{eqn:err_mmi} be denoted as $\calS$. Note that \eqref{eqn:y3in} implies that $y_2^n(j)$ is the $V$-shell and at least one other $\hatV$-shell  induced by an incorrect codeword. Also~\eqref{eqn:err_mmi} occurs if and only if the empirical conditional mutual information of an incorrect  codeword indexed by some $\tilm_j'\ne 1$ (i.e.,  $u^n(\tilm_j' |1 )$)  exceeds the nominal empirical  conditional mutual information induced by the true codeword $u^n(1 |1 )$. Thus, we have 
\begin{align}
\epsilon_\rmR&=\sum_{(V,\hatV) \in \calS}  \sum_{x_1^n \in \calT_{Q_{X_1|UX_2}}( u^n(1  | 1), x_2^n(1))} \frac{W^n(\calA_{V,V'}|x_1^n,x_2^n(1))}{|\calT_{Q_{X_1|UX_2}}( u^n(1 | 1), x_2^n(1))|} \label{eqn:uar_shell} \\
&\le\sum_{(V,\hatV) \in \calS}  \sum_{x_1^n \in \calT_{Q_{X_1|UX_2}}( u^n(1 | 1), x_2^n(1))} (n+1)^{|\calU||\calX_1| |\calX_2|}\exp(-nH(Q_{X_1|UX_2}| Q_{UX_2}))  W^n(\calA_{V,V'}|x_1^n,x_2^n(1))   \label{eqn:lower_bd_shell} \\
& = (n+1)^{|\calU||\calX_1| |\calX_2|} \sum_{(V,\hatV) \in \calS}  \sum_{x_1^n   \in \calT_{Q_{X_1|UX_2}}( u^n(1  | 1), x_2^n(1))   } Q_{X_1|UX_2}^n(x_1^n|u^n(1|1), x_2^n(1))   W^n(\calA_{V,V'}|x_1^n,x_2^n(1))   \label{eqn:prob_Shell} \\
& \le (n+1)^{|\calU||\calX_1| |\calX_2|} \sum_{(V,\hatV) \in \calS}  \sum_{x_1^n      } Q_{X_1|UX_2}^n(x_1^n|u^n(1|1), x_2^n(1))   W^n(\calA_{V,V'}|x_1^n,x_2^n(1))   \label{eqn:prob_Shell2} \\
& = (n+1)^{|\calU||\calX_1| |\calX_2|} \sum_{(V,\hatV) \in \calS}  W_{Y_2|UX_2}^n(\calA_{V,V'}|u^n(1|1),x_2^n(1))   \label{eqn:defWY_2}  
\end{align}
where \eqref{eqn:uar_shell} follows because $x_1^n(1,1|1)$ is generated uniformly at random from $\calT_{Q_{X_1|UX_2}}( u^n(1  | 1), x_2^n(1))$, \eqref{eqn:lower_bd_shell}  and  \eqref{eqn:prob_Shell} follow from Lemma~\ref{lem:types} and \eqref{eqn:defWY_2} follows from the definition of  $W_{Y_2|UX_2}$  in~\eqref{eqn:vir1}.


\iffalse
An error occurs in step~\eqref{eqn:decoder_j2} (conditioned on neighboring blocks being decoded correctly so $\check{m}_j'=\hatm_j'=1$) if and only if there exists $V,\hatV \in\scV_n( \calY_3; Q_{U X_2   X_1} )$ such that 
\begin{align}
y_3^n (j)\in\calA:= \calT_V(  u^n(1| 1), x_1^n(1,1|1),  x_2^n(1) )\bigcap\bigcup_{\tilm_j'' \ne 1} \calT_{\hatV}( u^n(1| 1) , x_1^n(\tilm_j'', 1|1),  x_2^n(1) )  \label{eqn:y3in}
\end{align}
 and
\begin{align}
I(Q_{X_1|U X_2},\hatV|Q_{U X_2})\ge I(Q_{X_1|U X_2},V|Q_{U X_2}) .\label{eqn:mmi}
\end{align}
Note that \eqref{eqn:y3in} implies that $y_3^n(j)$ is the $V$-shell and at least one other $\hatV$-shell  induced by an incorrect codeword. Also~\eqref{eqn:mmi} occurs iff the empirical conditional mutual information of an incorrect  codeword indexed by some $\tilm_j''\ne 1$ (i.e.,  $x_1^n(1, \tilm_j''|1)$), exceeds the nominal empirical  conditional mutual information induced by the true codeword $x_1^n(1, 1|1)$. Let $\calS \subset  \scV_n( \calY_3; Q_{U X_2   X_1} )^2$ be the set of all $(V,\hatV)$ pairs that satisfy \eqref{eqn:mmi}. Thus, we have
\begin{align}
\epsilon_{\rmD,2} &\le\sum_{(V,\hatV) \in \calS}W_{Y_3|U X_1 X_2 }^n \left(\calA   \,\big|\, u^n(1| 1), x_1^n(1,1|1),  x_2^n(1)\right) \\
&\le \sum_{(V,\hatV) \in \calS}  \exp(-nD(V\|W_{Y_3|U X_1 X_2}|Q_{U X_2 X_1} ) )  \exp(- n | I(Q_{X_1|U X_2},\hatV | Q_{U X_2})-R''  | ^+ )  \label{eqn:use_pack}  \\
&\le \sum_{V \in \scV_n( \calY_3; Q_{U,X_2,  X_1} )}  \exp(-nD(V\|W_{Y_3|U X_1 X_2}|Q_{U X_2 X_1} ) )  \exp(- n | I(Q_{X_1|U X_2},V | Q_{U X_2})-R''  | ^+ )   \label{eqn:higher_mi} \\
&\doteq \exp\left[-n\left(\min_{V :\calU\times \calX_2\times   \calX_1\to\calY_3}   D(V\|W_{Y_3|U X_1 X_2}|Q_{U X_2 X_1} )+ | I(Q_{X_1|U X_2},V | Q_{U X_2})-R''  | ^+  \right) \right], \label{eqn:final_decode}
% 2^{-n D(V||W_{Y_3|U,X_1,X_2}|Q_{U,X_2,X_1} ) } \nn\\*
% &\qquad\qquad \cdot\, 2^{- n |I(Q_{X_1|U X_2}, V|Q_{U X_2})-R'' |^+} .  %\\
% &\le\sum_{(V,\hatV)\in\calS} W_{Y_3|U,X_1,X_2}^n(\calT_V (u^n (m_{j}'|\hatm_{j-1}') , x_2^n(\hatm_{j-1}') ,  x_1^n(m_{j}', m_j''|m_{j-1}'))
\end{align}
where \eqref{eqn:use_pack} follows from \eqref{eqn:tvv}, Lemma~\ref{lem:types} and the fact that each sequence in a shell has equal probability, \eqref{eqn:higher_mi} follows from \eqref{eqn:mmi} and \eqref{eqn:final_decode} follows from the fact that the number of pairs  of conditional types is polynomial in $n$. \fi

Hence, we obtain  $\tilG(R'')$ in \eqref{eqn:G2} upon invoking continuity of  the exponents~\cite[Lem.\ 10.5]{Csi97} to replace types by distributions.  Note that since  $E_b(\Reff)$ is computed wrt the total blocklength $N=nb$, there is an additional factor of $1/b$ in~\eqref{eqn:pdf_lb}.
\end{proof}

\subsection{Proof of  Theorem~\ref{thm:expurate}} \label{prf:expu}
Before we prove the expurgated bound, we state a alternative version of Lemma~\ref{lem:packing_df}.
\begin{lemma}[Alternate  Packing Lemma for Expurgated Bound] \label{lem:spec}
Fix  $\delta>0$ and nonnegative numbers   $(R',R'')$ such that $R',R''>\delta$. For every $j \in [b]$, and for every joint type $Q_{X_2}\times Q_{U|X_2} \times Q_{X_1|U X_2} \in \scP_n(\calX_2\times\calU\times\calX_1)$ satisfying $H(Q_{X_2})<R'$, $H(Q_{U|X_2}|Q_{X_2}) < R'$ and $H(Q_{X_1 | U X_2} | Q_{U| X_2} Q_{X_2}) <R''$, there exists at least $\exp( n (R' - \delta) )$  sequences $(x_2^n(m_{j-1}'), u^n(m_j'|m_{j-1}')) \in \calT_{Q_{X_2} \times Q_{U|X_2}} $  and for every $(m_j',m_{j-1}') \in [\exp( n (R' - \delta) )]^2$ at least $\exp( n (R''-\delta))$ sequences $x_1^n(m_j', m_j''|m_{j-1}')\in \calT_{Q_{X_1|U X_2}}(  u^n(m_j'|m_{j-1}'), x_2^n(m_{j-1}'))$ such that for  all sufficiently large $n>n_1(\delta,b, |\calU|, |\calX_1|,  |\calX_2|, |\calY_2|, |\calY_3| )$, the sequences in the collection  satisfy  the following properties:

\begin{enumerate}
\item If $N(P_{U\tilU|X_2})$ denotes the number of  $\{u^n(\tilm_j' | m_{j-1}')\}_{\tilm_j'\ne m_j'}$  sequences with joint type $P_{U \tilU |X_2}$ given $x_2^n( m_{j-1}')$ with  $u^n(m_j' | m_{j-1}')$, then,
\begin{equation}
N(P_{U\tilU|X_2})\le \exp\left[  n  ( R'-I(Q_{U|X_2} , P_{\tilU|UX_2} |Q_{X_2} )  \right]. \label{eqn:expur_pack1}
\end{equation}
\item If $N( P_{UX_2 \tilU \tilX_2})$ denotes the number of sequences $\{(u^n(m_{j+1}' | \tilm_j'), x_2^n(\tilm_j'))\}_{\tilm_j'\ne m_j'}$ with joint type $P_{UX_2 \tilU \tilX_2}$ with $(u^n(m_{j+1}' | m_j'), x_2^n(m_j'))$, then,
\begin{equation}
N( P_{UX_2 \tilU \tilX_2})\le \exp\left[  n  ( R'-I(Q_{U X_2} , P_{\tilU\tilX_2|UX_2}  )  \right].
\end{equation}
\item If $N(P_{ X_1 \tilX_1| UX_2})$ denotes the number of $\{ x_1^n(m_j', \tilm_j''|m_{j-1}')\}_{\tilm_j''\ne m_j''}$  sequences with joint type $P_{ X_1 \tilX_1| UX_2}$ given $(u^n(m_j' | m_{j-1}'), x_2^n(m_{j-1}'))$ with $x_1^n(m_j', m_j''|m_{j-1}')$, then,
\begin{equation}
N(P_{ X_1 \tilX_1| UX_2})\le  \exp\left[  n  ( R'' - I(Q_{X_1|U X_2} , P_{\tilX_1|U X_2 X_1} |Q_{U X_2} )  \right].
\end{equation}
\end{enumerate}

%\begin{enumerate}
%\item For every $\{u^n(m_j' | m_{j-1}')\}_{m_j'}$ and triple of dummy random variables $X_2, U, \tilU$ whose joint distribution equals the joint type $P_{x_2^n(m_{j-1}'), u^n(m_j' | m_{j-1}'),  u^n( \tilm_j' | m_{j-1}') }=P_{X_2  U \tilU}$ for some  other sequence $u^n( \tilm_j' | m_{j-1}')$, $\tilm_j' \ne m_j'$,
%\begin{align}
%\left|\calT_{P_{\tilU|UX_2}}( u^n(m_j' | m_{j-1}'), x_2^n(m_{j-1}') ) \bigcap\calC  \right|\le \exp\left[  n  ( R'-I(Q_{U|X_2} , P_{\tilU|UX_2} |Q_{X_2} )  \right]. \label{eqn:expur_pack1}
%\end{align}
%\item For every $\{(u^n(m_{j+1}' | m_j'), x_2^n(m_j'))\}_{m_j'}$ and $4$-tuple of dummy random variables $U, X_2, \tilU, \tilX_2$ whose joint distribution equals the joint type $P_{ u^n(m_{j+1}' | m_j'), x_2^n(m_j'), u^n(m_{j+1}' | \tilm_j'), x_2^n(\tilm_j') } = P_{U X_2\tilU \tilX_2}$ for some other sequence  $(u^n(m_{j+1}' | \tilm_j'), x_2^n(\tilm_j'))$, $\tilm_j'\ne m_j'$,
%\begin{align}
%\left|\calT_{P_{\tilU\tilX_2|UX_2}}( u^n(m_{j+1}' | m_j'), x_2^n(m_j')  ) \bigcap\calC  \right|\le \exp\left[  n  ( R'-I(Q_{U X_2} , P_{\tilU\tilX_2|UX_2}  )  \right].
%\end{align}
%\item For every $\{ x_1^n(m_j', m_j''|m_{j-1}')\}_{m_j''}$ and $4$-tuple of dummy random variables $X_2,U, X_1, \tilX_1$ whose joint distribution equals the joint type $P_{ x_2^n(m_{j-1}'), u^n(m_j' | m_{j-1}'), x_1^n(m_j', m_j''|m_{j-1}'), x_1^n(m_j', \tilm_j''|m_{j-1}')}=P_{X_2 U X_1 \tilX_1}$ for some other sequence  $ x_1^n(m_j', \tilm_j''|m_{j-1}')$, $\tilm_j''\ne m_j''$, 
%\begin{align}
%\left|\calT_{ P_{\tilX_1|U X_2 X_1}  }(u^n(m_j' | m_{j-1}'), x_2^n(m_{j-1}'), x_1^n(m_j', m_j''|m_{j-1}') )\! \bigcap\!\calC  \right|\!\le\! \exp\left[  \! n  ( R''\!-\! I(Q_{X_1|U X_2} , P_{\tilX_1|U X_2 X_1} |Q_{U X_2} )  \right].
%\end{align}
%\end{enumerate}
\end{lemma}
This lemma  is a straightforward generalization as that for the  channel coding  case in  \cite[Lem.\ IV.1]{Csis00}. It can be proved   by random selection  and the main idea for \eqref{eqn:expur_pack1} is  to note that if $U^n(m_j'|m_{j-1}')$ and $U^n(\tilm_j'|m_{j-1}')$  are generated conditionally independently from the $Q_{U|X_2}$-shell given $x_2^n(m_{j-1}') \in \calT_{Q_{X_2}}$, the probability that they have joint type $P_{\tilU U |X_2}$ is   $\exp( -nI(Q_{U|X_2} , P_{\tilU|UX_2} |Q_{X_2} ))$ up to some polynomial. Observe that  if $R'< I(Q_{U|X_2} , P_{\tilU|UX_2} |Q_{X_2} ) $ in \eqref{eqn:expur_pack1}, the left-hand-side (LHS) of the inequality is zero since the right-hand-side (RHS) is smaller than one and the LHS must be integer-valued. We proceed to provide a sketch of the proof of Theorem~\ref{thm:expurate}.
\begin{proof}
The proof proceeds in a similar way to the proof of the random coding error exponent  in Section~\ref{prf:pdf}. Thus, we only delineate the key differences. The bound on the overall error probability is still bounded above as in~\eqref{eqn:union_bd}. We use the codebook provided  in Lemma~\ref{lem:spec}. Instead of using MMI decoding in~\eqref{eqn:relay_j}, the relay chooses $\check{m}_j$ to satisfy
\begin{equation}
\check{m}_j= \argmax_{m_j' \in [ \exp(n (R' -\delta) ) ] } W_{Y_2|UX_2}^n(y_2^n(j)| u^n(m_j'|m_{j-1}'), x_2^n(m_{j-1}') ),
\end{equation}
where $W_{Y_2|UX_2}$ is defined in \eqref{eqn:vir1}. In other words, conditional maximum-likelihood decoding is performed (conditioned on     the message in the previous block being decoded as $m_{j-1}'$). Similar conditional  maximum-likelihood  steps are done at the decoder. We now find the error exponent at the relay assuming $M_j'=M_{j-1}'=1$.  We have 
\begin{align}
\epsilon_\rmR \le\sum_{x_2^n(1) \in\calT_{Q_{X_2}}}\frac{1}{ | \calT_{Q_{X_2}}|}\sum_{\tilm_j'\ne 1} \sum_{y_2^n \in\calS(\tilm_j')} W_{Y_2|UX_2}^n(y_2^n |u^n(1|1), x_2^n(1) )
\end{align}
where $\calS(\tilm_j')$ is the set of sequences in $\calY_2^n$ that cause an error, i.e., 
\begin{equation}
\calS(\tilm_j'):= \left\{ y_2^n : W_{Y_2|UX_2}^n(y_2^n |u^n(\tilm_j'|1), x_2^n(1) )\ge  W_{Y_2|UX_2}^n(y_2^n |u^n(1|1), x_2^n(1) )   \right\}
\end{equation}
By using the definition of $\calS(\tilm_j')$, we have the following upper bound
\begin{align}
\epsilon_\rmR & \le\sum_{x_2^n(1) \in\calT_{Q_{X_2}}}\frac{1}{ | \calT_{Q_{X_2}}|}\sum_{\tilm_j'\ne 1} \sum_{y_2^n  } \sqrt{ W_{Y_2|UX_2}^n(y_2^n |u^n(1|1), x_2^n(1) )  W_{Y_2|UX_2}^n(y_2^n |u^n(\tilm_j'|1), x_2^n(1) )} \\
&= \sum_{\tilm_j'\ne 1} \exp\left( -n \bbE\left[ \rvd_{W_{Y_2|UX_2}} (U_1, U_{\tilm_j'}|X_2) \right]\right) \label{eqn:use_dist}
\end{align}
where \eqref{eqn:use_dist} invokes the definition of the conditional Bhattacharyya distance and the distribution of $(U_1, U_{\tilm_j'} ,  X_2)$ is the joint type of $(u^n(1|1), u^n(\tilm_j'|1), x_2^n(1))$. Now, let $N(P_{U \tilU|X_2})$ be the number of $u^n(\tilm_j'|1), \tilm_j'\ne 1$ sequences with conditional type  $P_{U \tilU|X_2}$ given $x_2^n(1)$.  This is the {\em type class enumerator}.  Note that the two marginals of $P_{U \tilU|X_2}$ have to be equal to $Q_{U|X_2}$. Then, by grouping the  $u^n(\tilm_j'|1), \tilm_j'\ne 1$ sequences  with the same conditional type together, we get
\begin{align}
\epsilon_\rmR &\le    \sum_{ P_{U \tilU|X_2}: P_{U|X_2}=P_{\tilU|X_2}=Q_{U|X_2} } N(P_{U \tilU|X_2}) \exp\left( -n \bbE\left[ \rvd_{W_{Y_2|UX_2}} (U, \tilU|X_2) \right]\right) 
\end{align}
Note that $N(P_{U \tilU|X_2})$ can be upper bounded using~\eqref{eqn:expur_pack1}. In particular, if the conditional type $P_{U \tilU|X_2}$ results in $R'<I(Q_{U|X_2} , P_{\tilU|UX_2} |Q_{X_2} )$, necessarily, $N(P_{U \tilU|X_2})=0$. Hence, we have
\begin{align}
\epsilon_\rmR &\le     \sum_{  \substack{ P_{U \tilU|X_2}:P_{U|X_2}=P_{\tilU|X_2}=Q_{U|X_2} \\  R'\ge I(Q_{U|X_2} , P_{\tilU|UX_2} |Q_{X_2} )}  } \exp\left[  n  ( R'-I(Q_{U|X_2} , P_{\tilU|UX_2} |Q_{X_2} )  \right] \exp\left( -n \bbE\left[ \rvd_{W_{Y_2|UX_2}} (U, \tilU|X_2) \right]\right)  \\
&\doteq \exp\left[- n\left( \min_{\substack{ P_{U \tilU|X_2}:P_{U|X_2}=P_{\tilU|X_2}=Q_{U|X_2} \\  R'\ge I(Q_{U|X_2} , P_{\tilU|UX_2} |Q_{X_2} )}  } \bbE\left[ \rvd_{W_{Y_2|UX_2}} (U, \tilU|X_2) \right]+ I(Q_{U|X_2} , P_{\tilU|UX_2} |Q_{X_2 } ) -R' \right)  \right].
\end{align}
This proves \eqref{eqn:Fx}. The other error exponents in \eqref{eqn:Gx} and \eqref{eqn:Gxtil} can be proven in the exact same fashion.% in view of the fact that the number of conditional types is polynomial.
\end{proof}

==> sphere_pack.tex <==
\section{An Upper Bound for the Reliability Function} \label{sec:sp}
\newcommand{\cmac}{\mathrm{C-MAC}}
\newcommand{\cbc}{\mathrm{C-BC}}

In this section, we state and prove an upper bound  on the reliability function defined in \eqref{eqn:tilE}. This is a sphere-packing-like bound~\cite{Haroutunian68} similar to that for  channels with full feedback proved by Haroutunian~\cite{Har77}. To do so, as is customary in the literature~\cite[Thm.~10.3, Ex.~10.36]{Csi97}, it is necessary to first prove a strong converse. In our setting, this means that all (sequences of) codes with rates above a certain rate result in error probabilities tending to one. We note that Behboodi and Piantanida~\cite{Beh11, Beh12} also claimed to have proved the strong converse above the cutset bound~\cite[Thm.~16.1]{elgamal}. They employed the general Verd\'u-Han~\cite[Lem.~4]{VH94} converse bound and the information spectrum method~\cite{Han10}. Here we provide an independent proof which results in a   weaker statement.\footnote{Unfortunately, the author was not able to verify the correctness  of all the  steps in the strong converse statement asserted by   Behboodi and Piantanida~\cite{Beh11, Beh12}. In particular, the strong converses stated in \cite[Thm.~3.3]{Beh11} and \cite[Thm.~3]{Beh12}  were not proved in full and some steps are not obvious. The complete strong converse argument appears in Behboodi's thesis~\cite{Behboodi} but in step (C.10), it is claimed that the final two $\mathrm{p}$-$\liminf$ terms are positive. This is not clear as the terms in the $\mathrm{p}$-$\liminf$ are not exactly mutual information rates and hence, positivity of the final two terms is not obvious. }

In Section~\ref{sec:strong_conv}, we state our strong converse which is proved in Section~\ref{sec:prf_strong_conv}. The upper bound on the reliability function is stated in Section~\ref{sec:sphere_pack}. Finally, this upper bound is proved in Section~\ref{sec:prf_sphere_pack}.

\subsection{Statement of the Strong Converse} \label{sec:strong_conv}
\begin{lemma}[Strong Converse] \label{lem:str_converse}
Every $(2^{nR} , n)$ code for the DM-RC (Definition~\ref{def:relay})  with average error probability not exceeding $\epsilon \in (0,1)$ must satisfy
\begin{equation}
R \le   \min\{ C_{\cmac}, C_{\cbc} \} + \theta_n \label{eqn:strong_con}.
\end{equation}
where 
\begin{align}
C_{\cmac} &:=\max_{P_{X_1 X_2}} I(X_1 X_2;Y_3) ,\label{eqn:cmac} \\
C_{\cbc}&:=\max_{P_{X_1 X_2}} I(X_1;Y_2Y_3|X_2) .\label{eqn:cbc}
\end{align}
are the capacities of the cooperative multiple-access channel  (C-MAC) and the cooperative broadcast channel (C-BC). The sequence  $\theta_n=O\big(\frac{1}{\sqrt{n}}\big)$ and the implied constant only depends on the cardinalities of the alphabets and error probability $\epsilon$. %Specifically,
%\begin{equation}
%\theta_n:=\sqrt{ (4.6\log |\calY_3|) n} + |\calX_1||\calX_2| \log (n+1) + \log \frac{2}{1-\epsilon}.
%\end{equation}
%%with $c(|\calY_3|,\epsilon)$ being only a function of $|\calY_3|$ and $\epsilon$.
\end{lemma}
Another way of interpreting Lemma~\ref{lem:str_converse} is the following: If the  rate of the code exceeds either   $C_{\cmac}$ or $C_{\cbc}$, the average error probability necessarily has to tend to one.  Note that this statement is weaker than that saying that above the cutset bound~\cite[Thm.~16.1]{elgamal}, all rates result in error probabilities tending to one. This is because the order of the min and max are swapped in \eqref{eqn:strong_con} relative to the cutset bound.  In general, our bound in \eqref{eqn:strong_con} is larger (looser) than that prescribed by  the cutset bound.

%The strong converse naturally leads to the following sphere-packing bound:
%\begin{theorem}[Sphere-Packing Bound for the Relay Channel]
%The reliability function, defined in \eqref{eqn:tilE}, is bounded from above as
%\begin{equation}
%\tilE(R)\le\max_{P_{X_1 X_2}}\min_{\substack{ V:\calX_1\times\calX_2\to\calY_3\\ I(P_{X_1X_2},V)\le R}}D(V\|W_{Y_3|X_1X_2}|P_{X_1 X_2}),
%\end{equation}
%where $W_{Y_3|X_1X_2}:\calX_1\times\calX_2\to\calY_3$ is the $\calY_3$-marginal of the DM-RC $W:\calX_1\times\calX_2\to\calY_2\times\calY_3$.
%\end{theorem}

\subsection{Proof of the Strong Converse } \label{sec:prf_strong_conv}
We only prove the strong converse statement in full for $C_{\cmac}$. The statement for $C_{\cbc}$ follows very similarly by regarding $X_2^n$ as noncausl side information at the transmitter and receiver. See \cite{TomTan13} for an analogous converse for channel coding with noncausal state information at both terminals. 

Before we prove the strong converse for $C_{\cmac}$, we start with a few important definitions from~\cite{TomTan12}. Let $P,Q\in\scP(\calZ)$ be two probability measures  and assume that $P$ is absolutely continuous with respect to $Q$. Let the {\em $\epsilon$-hypothesis testing divergence} be defined as 
\begin{equation} \label{eqn:def_Dh}
D_\rmh^\epsilon(P\| Q):=\sup\left\{ R\in\bbR: \exists\, \delta:\calZ\to [0,1] , \bbE_Q[\delta(Z)]\le (1-\epsilon)2^{-R}, \bbE_P[\delta(Z)]\ge 1-\epsilon\right\}.
\end{equation}
Also define the {\em $\epsilon$-information spectrum divergence} as 
\begin{equation} \label{eqn:def_Ds}
D_\rms^\epsilon(P\| Q):=\sup\left\{ R\in\bbR:  P \left(\log  \frac{P(Z)}{Q(Z)}\le R  \right)\le \epsilon\right\},
\end{equation}
where $Z$ has distribution $P$. 
Note that in \eqref{eqn:def_Dh}, $\delta:\calZ\to [0,1]$ represents  a randomized hypothesis test between $P$ and $Q$.  Now we can state a non-asymptotic  upper bound on the code size for relay channels that will eventually lead to the strong converse statement of Lemma~\ref{lem:str_converse}.

\begin{lemma}[Bound on the Code Size for DM-RCs] \label{lem:code_size}
Every $(2^{nR}, n)$ code for the DM-RC (Definition~\ref{def:relay}) with average error probability not exceeding $\epsilon \in (0,1)$ must satisfy
\begin{equation}
nR\le  \inf_{\eta\in (0,1-\epsilon)}\inf_{Q\in\scP(\calY_3^n)}\sup_{(x_1^n, x_2^n)\in\calX_1^n\times\calX_2^n} D_\rms^{\epsilon+\eta}(W_{Y_3|X_1X_2}^n(\fndot|x_1^n, x_2^n) \| Q)+\log\frac{1}{\eta}. \label{eqn:bound_code_size}
\end{equation}
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lem:code_size}]
For any DM-RC, we claim that the Markov chain 
\begin{equation}
M\longrightarrow (X_1^n, X_2^n) \longrightarrow Y_3^n\longrightarrow \hatM \label{eqn:mc}
\end{equation}
holds.  Let us justify \eqref{eqn:mc}. The joint distribution of $(M, X_1^n, X_2^n, Y_2^n, Y_3^n, \hatM)$ given the encoder  $f:\calM\to\calX_1^n$, the sequence of relay encoders $g_i:\calY_2^{i-1}\to\calX_2, i \in [n]$ and the decoder $\varphi:\calY_3^n\to\calM$ is 
\begin{equation}
P_{MX_1^n  X_2^n  Y_2^n  Y_3^n  \hatM}(m, x_1^n, x_2^n, y_2^n ,y_3^n,\hatm):=\frac{\bone\{x_1^n=f(m)\}}{2^{nR}}\prod_{i=1}^n W(y_{2i},y_{3i}| f(m)_i, g_i(y_2^{i-1})) \bone\{\varphi(y_3^n )=\hatm\}.
\end{equation}
Marginalizing over $y_2^n$ yields
\begin{equation}
P_{MX_1^n  X_2^n     Y_3^n  \hatM}(m, x_1^n, x_2^n ,y_3^n,\hatm)=\phi_1(m)\phi_2(x_1^n,m)\phi_3(x_1^n , x_2^n ,y_3^n)\phi_4(y_3^n,\hatm).\end{equation}
for some functions $\phi_j,j=1,\ldots, 4$ implying the Markov condition in \eqref{eqn:mc} by the Hammersley-Clifford theorem for undirected graphical models~\cite{Lau96}.  This Markov chain induces the joint distribution $P_{M X_1^n X_2^n Y_3^n \hatM}$.

  Let $Q$ be any distribution on $\scP(\calY_3^n)$. Due to the data-processing inequality for $D_\rmh^\epsilon$, we have 
\begin{equation} \label{eqn:dpi}
D_\rmh^\epsilon(P_{X_1^n X_2^n }\times W_{Y_3|X_1 X_2}^n \|P_{X_1^n X_2^n  }\times Q)\ge D_{\rmh}^\epsilon(P_{M \hatM }\|P_M  \times Q_{\hatM})
\end{equation}
where $Q_{\hatM}$ is the distribution induced by the decoder's operation  on  $Y_3^n$.  Consider the non-randomized test  $\delta$ on $\calZ:=\calM\times\calM$ given by 
\begin{equation}
\delta(m,\hatm):=\bone\{ m=\hatm\}
\end{equation}
This test satisfies 
\begin{align}
\bbE_{P_{M \hatM}}[\delta(M, \hatM)]&=\bbP(\hatM=M)\ge 1-\epsilon,\\
\bbE_{P_{M} \times Q_{\hatM}}[\delta(M, \hatM)]&=\frac{1}{2^{nR}}
\end{align}
As a result, by the definition of the $\epsilon$-hypothesis testing divergence,
\begin{equation}
D_{\rmh}^\epsilon(P_{M \hatM }\|P_M \times  Q_{\hatM})\ge nR+\log(1-\epsilon) .
\end{equation}
Combining with \eqref{eqn:dpi} yields,
\begin{equation}
D_\rmh^\epsilon(P_{X_1^n X_2^n }\times W_{Y_3|X_1 X_2}^n \|P_{X_1^n X_2^n  }\times Q)\ge nR+\log(1-\epsilon) .
\end{equation}
Furthermore, by applying \cite[Lems.~2 and 4]{TomTan12}, we have 
\begin{align}
&\sup_{x_1^n,x_2^n}D_\rms^{\epsilon+\eta}(  W_{Y_3|X_1 X_2}^n (\fndot|x_1^n, x_2^n) \|   Q)\nn\\
&\quad \ge D_\rms^{\epsilon+\eta}(  P_{X_1^n X_2^n  }\times W_{Y_3|X_1 X_2}^n (\fndot|x_1^n, x_2^n) \| P_{X_1^n X_2^n  }\times Q)\\
&\quad \ge D_\rmh^{\epsilon}(  P_{X_1^n X_2^n  }\times W_{Y_3|X_1 X_2}^n (\fndot|x_1^n, x_2^n) \| P_{X_1^n X_2^n  }\times Q)-\log\frac{1-\epsilon}{\eta}\\
&\quad \ge nR-\log\frac{1}{\eta}.
\end{align}
Optimizing over $\eta \in (0,1-\epsilon)$ and $Q\in\scP(\calY_3^n)$ yields the bound \eqref{eqn:bound_code_size} as desired.
\end{proof}
We now use Lemma~\ref{lem:code_size} to prove the strong converse.
\begin{proof}[Proof of Lemma~\ref{lem:str_converse}] The main idea is to choose a judicious $Q$ in \eqref{eqn:bound_code_size}. We take 
\begin{equation}
Q(y_3^n):= \frac{1}{|\scP_n(\calX_1\times\calX_2)|}\sum_{P \in \scP_n(\calX_1\times\calX_2)} \prod_{i=1}^n PW_{Y_3|X_1 X_2} (y_{3i}) \label{eqn:choice_Q}
\end{equation}
where the marginal distribution $ PW_{Y_3|X_1 X_2} \in\scP(\calY_3)$ is defined as
\begin{equation}
 PW_{Y_3|X_1 X_2} (y_3):=\sum_{x_1, x_2} P(x_1,x_2)W_{Y_3|X_1 X_2} (y_3|x_1,x_2).
\end{equation}
Thus $Q$ is a mixture of output distributions induced by input joint types on $\calX_1\times \calX_2$. Now take $\eta:=(1-\epsilon)/2>0$. Then, we upper bound $D_\rms^{\epsilon+\eta}(W_{Y_3|X_1 X_2}^n  (\fndot|x_1^n, x_2^n) \| Q)$ for every sequence $(x_1^n, x_2^n)$ with the choice of $Q$ in \eqref{eqn:choice_Q}. It is clear from the definition of the $\epsilon$-information spectrum divergence that 
\begin{align}
&D_\rms^{\epsilon+\eta}(W_{Y_3|X_1 X_2}^n  (\fndot|x_1^n, x_2^n) \| Q)\nn\\
&\quad \le D_\rms^{\epsilon+\eta}(W_{Y_3|X_1 X_2}^n  (\fndot|x_1^n, x_2^n) \| (P_{x_1^n, x_2^n}W_{Y_3|X_1 X_2})^n ) + \log|\scP_n(\calX_1\times\calX_2)|\\
&\quad \le D_\rms^{\epsilon+\eta}(W_{Y_3|X_1 X_2}^n  (\fndot|x_1^n, x_2^n) \| (P_{x_1^n, x_2^n}W_{Y_3|X_1 X_2})^n ) +  |\calX_1||\calX_2| \log (n+1). \label{eqn:num_jt_types}
\end{align}
What we have done is to simply pick out the output distribution that corresponds to the  joint type of $(x_1^n, x_2^n)$. By applying Chebyshev's inequality to the $\epsilon$-information spectrum divergence,
\begin{align}
&D_\rms^{\epsilon+\eta}(W_{Y_3|X_1 X_2}^n  (\fndot|x_1^n, x_2^n) \| (P_{x_1^n, x_2^n}W_{Y_3|X_1 X_2})^n )\nn\\
 &\quad \le n I(P_{x_1^n, x_2^n}, W_{Y_3|X_1 X_2}) + \sqrt{\frac{n V(P_{x_1^n, x_2^n}, W_{Y_3|X_1 X_2})}{1-\epsilon-\eta}} \label{eqn:dispersion}\\
 &\quad \le nC_{\cmac}+ \sqrt{\frac{n V(P_{x_1^n, x_2^n}, W_{Y_3|X_1 X_2})}{1-\epsilon-\eta}} \label{eqn:use_cmac}\\
&\quad \le nC_{\cmac}+ \sqrt{  \frac{2( 2.3n\log |\calY_3|)}{1-\epsilon}}\label{eqn:uniform_bd_dispersion}
\end{align}
where in \eqref{eqn:dispersion}, $V(P,W):=\sum_x P(x)\var_{W(\fndot|x)}[\log \frac{W(\fndot|x)}{PW(\fndot)} - D(W(\fndot|x) \| PW(\fndot))]^2$ is the conditional information variance and \eqref{eqn:use_cmac} uses the definition  of $C_{\cmac}$  in \eqref{eqn:cmac}  and~\eqref{eqn:uniform_bd_dispersion} uses the definition of  $\eta$ as well as the uniform bound on the  information variance  in \cite[Rmk.~3.1.1]{Han10}. Uniting \eqref{eqn:num_jt_types} with \eqref{eqn:uniform_bd_dispersion} yields the strong converse for $C_{\cmac}$.
\end{proof}

\subsection{The Upper Bound on the Reliability Function}\label{sec:sphere_pack}

Equipped with the strong converse statement in Lemma~\ref{lem:str_converse}, it is  now relatively straightforward to prove the upper  bound on the reliability function using the Haroutunian~\cite{Har77} technique for proving a lower bound to error probability for channels with full feedback. Before we commence, define the function 
\begin{equation}
\rvC(V):=\min\left\{ \max_{P_{X_1X_2}} I(P_{X_1X_2}, V_{Y_3|X_1X_2}) ,\max_{P_{X_1X_2}} I(P_{X_1|X_2}, V|P_{X_2}) \right\},
\end{equation}
where $V$ represents a  transition matrix from $\calX_1\times\calX_2$ to $\calY_2\times \calY_3$ and $V_{Y_3|X_1X_2}$ is its $\calY_3$-marginal.

\begin{theorem}[Upper Bound on the Reliability Function] \label{thm:upper}
We have the following upper bound on $E(R)$:
\begin{align}
E(R)\le E^{+}(R) &:=\min_{ \substack{ V : \calX_1\times\calX_2\to\calY_2\times \calY_3 \\ \rvC(V)\le R}} \max_{P_{X_1X_2}}D( V\| W| P_{X_1X_2}) \label{eqn:ub_rel}\\
& =\min_{ \substack{ V : \calX_1\times\calX_2\to\calY_2\times \calY_3 \\ \rvC(V)\le R}}  \max_{x_1, x_2} D( V(\fndot,\fndot| x_1, x_2)\| W(\fndot,\fndot| x_1, x_2) ) \label{eqn:ub_rel2}.
\end{align}
\end{theorem}
Clearly, for all $R<\min\{ C_{\cmac}, C_{\cbc}\}$, the upper bound $E^{+}(R)$ is positive.   

We expect that the upper bound is extremely loose relative to the achievability  bounds prescribed by Theorems~\ref{thm:pdf} and~\ref{thm:cf}. This is because (i) the cutoff rates are different---in general the PDF and CF bounds do not match the cutset bound unless the DM-RC has some additional structure~\cite[Ch.~16]{elgamal} and (ii) achievability theorems leverage on block-Markov coding and hence the exponents are attenuated by the number of blocks  $b$ causing huge delay when $b$ is large. This  factor is not present in Theorem~\ref{thm:upper}.

One obvious improvement is to strengthen the strong converse statement in Lemma~\ref{lem:str_converse}. Another method to strengthen the exponent is to consider codes with limited (finite) memory, i.e., there exists some integer $l\ge 1$ (that does not depend on $n$) such that $g_i(y_2^{i-1}) = g_i (y_{2, i-l}^{i-1})$. Under this analogous assumption for the discrete memoryless channel (DMC), Como and Nakibo\u{g}lu~\cite{Como} showed that the sphere-packing bound is an upper bound for DMCs with full feedback, thus improving on Haroutunian's result~\cite{Har77}.


\subsection{Proof of Theorem~\ref{thm:upper}}\label{sec:prf_sphere_pack}
\begin{proof}
Let $V : \calX_1\times\calX_2\to\calY_2\times \calY_3$ be such that $\rvC(V)\le R$.  Let $\delta>0$ be an arbitrarily small number.  Then by the strong converse we proved earlier (Lemma~\ref{lem:str_converse}), the average error probability assuming the DM-RC is channel $V$, denoted as $\rmP_{\rme}(V)$, satisfies
\begin{equation}
\rmP_{\rme}(V)\ge 1-\delta. \label{eqn:Vge}
\end{equation}
Because there is ``feedback'' in the form of the signal $Y_2^n$, we cannot apply the standard Haroutunian change-of-measure technique in \cite{Haroutunian68}. Also see \cite[Thm.~10.1]{Csi97}. Thus,  we follow the proof strategy in Palaiyanur~\cite[Lem.~18]{Palai11}. For a given  channel $W: \calX_1\times\calX_2\to\calY_2\times \calY_3$ and  code with encoding functions $f, g_i, i\in [n]$ and decoding regions $\calD_m,m\in\calM$,  define $\bbP_W((Y_2^n,Y_3^n) = (y_2^n,y_3^n)|M=m)$ to be the probability that $(Y_2^n,Y_3^n) = (y_2^n,y_3^n)$ when message $m$ is sent, i.e., 
\begin{equation}
\bbP_W((Y_2^n,Y_3^n) = (y_2^n,y_3^n)|M=m):=\prod_{i=1}^n W(y_{2i}, y_{3i} | f(m)_i, g_i(y_2^{i-1}) ).
 \end{equation} 
Let $g^n:\calY_2^n\to\calX_2^n$ denote the concatenation of all the relay encoders, i.e., $g^n(y_2^n) := (x_2^*, g_2(y_2^1),g_3(y_2^2), \ldots, g_n(y_2^{n-1}))$ where $x_2^*$ is any fixed symbol in $\calX_2$.  Also for a type $P\in\scP_n(\calX_1,\times\calX_2)$ and conditional type $U\in\scV_n(\calY_2\times\calY_3;P)$, define the set 
\begin{equation}
\calB(m, P, U) := \left\{(y_2^n, y_3^n) : (f(m), g^n(y_2^n)) \in\calT_P , y_3^n \in\calT_U(f(m), g^n(y_2^n)) \right\}
\end{equation}
From the definition of $\rmP_{\rme}(W)$, we have
\begin{align}
\rmP_{\rme}(W) &= \frac{1}{|\calM|}\sum_{m\in\calM}\bbP_W(Y_3^n \in\calD_m^c| M=m) \\
&= \frac{1}{|\calM|}\sum_{m\in\calM} \sum_{ \substack{ P\in\scP_n(\calX_1\times\calX_2) \\  U \in\scV_n(\calY_2\times\calY_3;P)} } \sum_{\substack{ (y_2^n,y_3^n) \in\calB(m, P, U) \\ y_3^n \in\calD_m^c}}  \bbP_W((Y_2^n,Y_3^n) =(y_2^n,y_3^n)| M=m) \\
&= \frac{1}{|\calM|}\sum_{m\in\calM} \sum_{ \substack{ P\in\scP_n(\calX_1\times\calX_2) \\  U \in\scV_n(\calY_2\times\calY_3;P)} } \sum_{\substack{ (y_2^n,y_3^n) \in\calB(m, P, U) \\ y_3^n \in\calD_m^c}} \bbP_V((Y_2^n,Y_3^n) =(y_2^n,y_3^n)| M=m) \nn\\
&\qquad\qquad\qquad \times \prod_{i=1}^n \frac{W(y_{2i}, y_{3i} | f(m)_i, g_i(y_2^{i-1})) }{V(y_{2i}, y_{3i} | f(m)_i, g_i(y_2^{i-1})) }\\
&= \frac{1}{|\calM|}\sum_{m\in\calM} \sum_{ \substack{ P\in\scP_n(\calX_1\times\calX_2) \\  U \in\scV_n(\calY_2\times\calY_3;P)} } \sum_{\substack{ (y_2^n,y_3^n) \in\calB(m, P, U) \\ y_3^n \in\calD_m^c}}  \bbP_V((Y_2^n,Y_3^n) =(y_2^n,y_3^n)| M=m)  \nn\\
 &\qquad\qquad\qquad \times \prod_{x_1, x_2, y_2, y_3} \left(\frac{W(y_2, y_3|x_1, x_2)}{V(y_2, y_3|x_1, x_2)} \right)^{nP(x_1, x_2)U(y_2,y_3|x_1, x_2)} 
\end{align}
where the last line follows from the definition of the set $\calB(m, P, U)$. Continuing, we have 
\begin{align}
\frac{\rmP_{\rme}(W)}{\rmP_{\rme}(V)} &\ge \frac{1}{|\calM|}\sum_{m\in\calM} \sum_{ \substack{ P\in\scP_n(\calX_1\times\calX_2) \\  U \in\scV_n(\calY_2\times\calY_3;P)} } \sum_{\substack{ (y_2^n,y_3^n) \in\calB(m, P, U) \\ y_3^n \in\calD_m^c}} \frac{\bbP_V((Y_2^n,Y_3^n) =(y_2^n,y_3^n)| M=m)}{\rmP_{\rme}(V)}  \nn\\
 & \qquad\qquad\qquad \times \exp\left( -n   \sum_{x_1, x_2, y_2, y_3} P(x_1,x_2) U(y_2,y_3|x_1,x_2)\log\frac{V(y_2,y_3|x_1,x_2)}{W(y_2,y_3|x_1,x_2)}\right) \\
 & \ge\exp\Bigg[ -n \bigg(  \frac{1}{|\calM|}\sum_{m\in\calM} \sum_{ \substack{ P\in\scP_n(\calX_1\times\calX_2) \\  U \in\scV_n(\calY_2\times\calY_3;P)} } \sum_{\substack{ (y_2^n,y_3^n) \in\calB(m, P, U) \\ y_3^n \in\calD_m^c}} \frac{\bbP_V((Y_2^n,Y_3^n) =(y_2^n,y_3^n)| M=m)}{\rmP_{\rme}(V)}   \nn\\ 
 & \qquad\qquad\qquad \times     \sum_{x_1, x_2, y_2, y_3} P(x_1,x_2) U(y_2,y_3|x_1,x_2)\log\frac{V(y_2,y_3|x_1,x_2)}{W(y_2,y_3|x_1,x_2)}\bigg)
 \Bigg] \label{eqn:changetoV} .
\end{align}
The last step \eqref{eqn:changetoV}  follows from the convexity of $t\mapsto \exp(t)$.  Now the idea is to approximate $U$ with $V$. For this purpose, define the ``typical'' set 
\begin{equation}
\calJ_\gamma(V) := \left\{ (P,U)  : \sum_{x_1, x_2, y_2, y_3} P(x_1, x_2) |U(y_2,y_3|x_1, x_2)-V(y_2,y_3|x_1, x_2)|\le\gamma\right\}.
\end{equation}
Also define the finite constant 
\begin{equation}
\kappa_V := \max_{x_1, x_2, y_2, y_3: V(y_2,y_3|x_1,x_2) > 0 } - \log V(y_2,y_3|x_1,x_2).
\end{equation}
For $(P,U)\in\calJ_\gamma(V)$, it is easy to check by using the definition of $D(V\|W|P)$ that 
\begin{equation}
  \sum_{x_1, x_2, y_2, y_3} P(x_1,x_2) U(y_2,y_3|x_1,x_2)\log\frac{V(y_2,y_3|x_1,x_2)}{W(y_2,y_3|x_1,x_2)}\le D(V\|W|P) + \gamma\max\{ \kappa_V,\kappa_W\} .\label{eqn:inJ}
 \end{equation}
 Thus, we have 
\begin{align}
T &:= \frac{1}{|\calM|}\sum_{m\in\calM} \sum_{ \substack{ P\in\scP_n(\calX_1\times\calX_2) \\  U \in\scV_n(\calY_2\times\calY_3;P) \\ (P,U) \in\calJ_\gamma(V)} } \sum_{\substack{ (y_2^n,y_3^n) \in\calB(m, P, U) \\ y_3^n \in\calD_m^c}} \frac{\bbP_V((Y_2^n,Y_3^n) =(y_2^n,y_3^n)| M=m)}{\rmP_{\rme}(V)}   \nn\\ 
 & \qquad\qquad\qquad \times     \sum_{x_1, x_2, y_2, y_3} P(x_1,x_2) U(y_2,y_3|x_1,x_2)\log\frac{V(y_2,y_3|x_1,x_2)}{W(y_2,y_3|x_1,x_2)} \\
 &\le \left[ \max_P D(V\|W|P) + \gamma\max\{ \kappa_V,\kappa_W\} \right] \nn\\
 & \qquad\qquad\qquad \times   \frac{1}{|\calM|}\sum_{m\in\calM}\sum_{ \substack{ P\in\scP_n(\calX_1\times\calX_2) \\  U \in\scV_n(\calY_2\times\calY_3;P) \\ (P,U) \in\calJ_\gamma(V) } } \sum_{\substack{ (y_2^n,y_3^n) \in\calB(m, P, U) \\ y_3^n \in\calD_m^c}} \frac{\bbP_V((Y_2^n,Y_3^n) =(y_2^n,y_3^n)| M=m)}{\rmP_{\rme}(V)}   \\
  &\le \left[ \max_P D(V\|W|P) + \gamma\max\{ \kappa_V,\kappa_W\} \right] \nn\\
 & \qquad\qquad\qquad \times   \frac{1}{|\calM|}\sum_{m\in\calM}\sum_{ \substack{ P\in\scP_n(\calX_1\times\calX_2) \\  U \in\scV_n(\calY_2\times\calY_3;P) } }  \frac{\bbP_V((Y_2^n,Y_3^n)  \in \calB(m,P,U) , Y_3^n \in \calD_m^c| M=m)}{\rmP_{\rme}(V)}   \\
  &= \left[ \max_P D(V\|W|P) + \gamma\max\{ \kappa_V,\kappa_W\} \right]   \frac{1}{|\calM|}\sum_{m\in\calM} \frac{\bbP_V(Y_3^n\in\calD_m^c | M=m)}{\rmP_{\rme}(V)}   \\
  & =\max_P D(V\|W|P) + \gamma\max\{ \kappa_V,\kappa_W\}.\label{eqn:inJ2}
\end{align}
The last step follows from the definition of the average error probability $\rmP_{\rme}(V)$. For $(P,U)\notin\calJ_\gamma(V)$, it is also easy to check using \cite{Weiss03} that 
\begin{equation}
\sum_{  \substack{  P\in\scP_n(\calX_1\times\calX_2) \\  U \in\scV_n(\calY_2\times\calY_3;P)  \\ (P,U) \notin\calJ_\gamma(V) }} \bbP_V((Y_2^n,Y_3^n)\in \calB(m,P,U) | M=m) \le (n+1)^{|\calX_1| |\calX_2| |\calY_2| |\calY_3| } \exp\left(-n\frac{\gamma^2}{2} \right). \label{eqn:notinJ}
\end{equation}
As such,
\begin{align}
S &:= \frac{1}{|\calM|}\sum_{m\in\calM} \sum_{ \substack{ P\in\scP_n(\calX_1\times\calX_2) \\  U \in\scV_n(\calY_2\times\calY_3;P) \\ (P,U) \notin\calJ_\gamma(V)} } \sum_{\substack{ (y_2^n,y_3^n) \in\calB(m, P, U) \\ y_3^n \in\calD_m^c}} \frac{\bbP_V((Y_2^n,Y_3^n) =(y_2^n,y_3^n)| M=m)}{\rmP_{\rme}(V)}   \nn\\ 
 & \qquad\qquad\qquad \times     \sum_{x_1, x_2, y_2, y_3} P(x_1,x_2) U(y_2,y_3|x_1,x_2)\log\frac{V(y_2,y_3|x_1,x_2)}{W(y_2,y_3|x_1,x_2)} \\
& \le\frac{\kappa_W}{\rmP_{\rme}(V) }  (n+1)^{|\calX_1| |\calX_2| |\calY_2| |\calY_3| } \exp\left(-n\frac{\gamma^2}{2} \right).\label{eqn:notinJ2}
\end{align}
Combining \eqref{eqn:changetoV}, \eqref{eqn:inJ2} and \eqref{eqn:notinJ2}, we conclude that 
\begin{equation}
\frac{\rmP_{\rme}(W)}{\rmP_{\rme}(V)}\ge\exp[-n(T+S)]\ge \exp\left[-n \left( \max_P D(V\|W|P) + \xi(n,\gamma)\right) \right]
\end{equation}
where  
\begin{equation}
\xi(n,\gamma):=\gamma\max\{ \kappa_V,\kappa_W\}+\frac{\kappa_W}{\rmP_{\rme}(V) }  (n+1)^{|\calX_1| |\calX_2| |\calY_2| |\calY_3| } \exp\left(-n\frac{\gamma^2}{2} \right).
\end{equation}
Choosing the channel $V$ to achieve the minimum in \eqref{eqn:ub_rel} and applying~\eqref{eqn:Vge} yields
\begin{align}
\rmP_{\rme}(W)\ge (1-\delta)\exp\left[-n \left( E^+(R) + \xi(n,\gamma)\right) \right].
\end{align}
Thus, by taking the limit of the normalized logarithm,
\begin{equation}
\liminf_{n\to\infty}\frac{1}{n}\log \frac{1}{\rmP_{\rme}(W)}\le E^+(R) + \gamma\max\{ \kappa_V,\kappa_W\}.
\end{equation}
Now take $\gamma\downarrow 0$. This completes the proof.
 \end{proof}
